Risk Set Matched Difference-in-Differences for the Analysis of Effect Modification in an Observational Study on the Impact of Gun Violence on Health Outcomes

Gun violence is a major source of injury and death in the United States. However, relatively little is known about the effects of firearm injuries on survivors and their family members and how these effects vary across subpopulations. To study these questions and, more generally, to address a gap in the causal inference literature, we present a framework for the study of effect modification or heterogeneous treatment effects in difference-in-differences designs. We implement a new matching technique, which combines profile matching and risk set matching, to (i) preserve the time alignment of covariates, exposure, and outcomes, avoiding pitfalls of other common approaches for difference-in-differences, and (ii) explicitly control biases due to imbalances in observed covariates in subgroups discovered from the data. Our case study shows significant and persistent effects of nonfatal firearm injuries on several health outcomes for those injured and on the mental health of their family members. Sensitivity analyses reveal that these results are moderately robust to unmeasured confounding bias. Finally, while the effects for those injured vary largely by the severity of the injury and its documented intent, for families, effects are strongest for those whose relative's injury is documented as resulting from an assault, self-harm, or law enforcement intervention.

==> matchDID_supp_sec1.tex <==
 \subsection{Details on Risk Set Matching}
Risk set matching \citep{LiYunfeiPaul2001BRSM} matches each newly treated unit at time $t$ with controls who are not yet treated based on covariate information up to time $t$. 
Once a control is used in a match, it is discarded from the pool of potential controls for future-treated units.
This structure enables the use of traditional methods for randomization and sensitivity analysis, as in \cite{RN55} via the following model for the hazards of treatment at time $t$ for unit $i$:
\begin{align}
\label{eq_hazards}
h_{tij} = \lim_{\delta \to 0} \mathbb{P}\left(t + \delta \geq Z_{ij} \geq t | Z_{ij} \geq t\right) / \delta = \exp\left(\xi\left(\bm{x}_{tij}(\infty)\right) + \gamma u_{tij} \right)
\end{align}
where $u_{tij}$ is an unmeasured variable, $\xi(\cdot)$ is an arbitrary function, and $\gamma \in \mathbb{R}$.
Thus, the hazards of treatment at time $t$ is a function of the control potential covariates (which, by Assumption 2, are observed because the units are not yet treated) and unmeasured confounders, where these two sets of variables do not interact.
When $\gamma = 0$, there is no unmeasured confounding (i.e., as in Assumption 4), this places no restrictions on the relationship between the potential covariates and the hazards.
The no-interaction relationship between the unmeasured variables and the other covariates enables the use of conventional sensitivity analyses for unmeasured confounding \citep{RN6}.

Under \eqref{eq_hazards}, we have:
\begin{align}
\label{eq_assignment}
\mathbb{P}\left(\bm{W} = \bm{w} | \mathcal{D} \right) = \prod_{i = 1}^{I} \dfrac{\exp\left(\gamma \sum_{j=1}^{n_i} w_{ij} u_{ij}\right)}{\sum_{j=1}^{n_i} \exp \left(\gamma u_{ij}\right)}
\end{align}
where $\bm{W} = (W_{11}, ..., W_{1n_1}, ..., W_{In_I})$ and $\mathcal{D}$ denotes the matching design (i.e., the matched sets).
